Bridging the Gap: A Survey and Classification of Research-Informed Ethical Hacking Tools

The majority of Ethical Hacking (EH) tools utilised in penetration testing are developed by practitioners within the industry or underground communities. Similarly, academic researchers have also contributed to developing security tools. However, there appears to be limited awareness among practitioners of academic contributions in this domain, creating a significant gap between industry and academia's contributions to EH tools. This research paper aims to survey the current state of EH academic research, primarily focusing on research-informed security tools. We categorise these tools into process-based frameworks (such as PTES and Mitre ATT\&CK) and knowledge-based frameworks (such as CyBOK and ACM CCS). This classification provides a comprehensive overview of novel, research-informed tools, considering their functionality and application areas. The analysis covers licensing, release dates, source code availability, development activity, and peer review status, providing valuable insights into the current state of research in this field.

==> tasks.tex <==
\section*{Tasks for contributors (To be removed in final version)}

\begin{itemize}
	\item Identify at least 25 tools satisfying ALL the criteria described below. (\textit{Methodology} \ref{sec:Methodology}). Save the data (all fields) in an Excel template, and produce a file .bib file with the list. Exclude tools already existing in the current list.
	\url{https://liveteesac-my.sharepoint.com/:x:/r/personal/p_modesti_tees_ac_uk/_layouts/15/Doc.aspx?sourcedoc=%7BFAD0DE58-8F9D-410A-87FD-350489B6BEE8%7D&file=Research%20Project%20Papers.xlsx}
	
	We are considering tools that satisfy the following criteria:
	
	\begin{itemize}
		\item There is at least one "good" peer-reviewed paper presenting the tool architecture and functionalities.
		\item The tool has a potential to be used in an offensive context, e.g. ethical hacking, even if authors do not state that explicitly, as the tool could have been developed for another purpose (e.g. software testing, supporting software or system development)
		\item The authors of the papers have designed/developed the tool	
		\item The tool has been developed within an academic/research project: this excludes any tools developed primarily as practitioner tool.
		\item Some authors are affiliated to universities or public research centres.
		\item Ideally, the tool is open source, and the source code (or distribution package) is freely available.
		\item The tool is not part of Kali Linux (or immediately installable on Kali Linux or similar distribution)
		\item Published in the last decade (2013 and later)
		\item Exclude tools that merely aggregate result from practitioner tools.
	\end{itemize}
	
	
	\item Contribute to the classification of the tools, within the context of Ethical Hacking, and double check the classification itself.
	\item Write a description of a number of tools in Section \textit{Review of Research and Tools} \ref{sec:Review-of-Research} and discuss them.
	\item Write some sections of the paper (either leading it or contributing).
	\item Contribute to the \textit{List of Abbreviations} \ref{app:abbreviations}.
	\item Quality check, proofreading and finalisation of the paper.
	\item Shared folder: \url{https://liveteesac-my.sharepoint.com/:f:/g/personal/p_modesti_tees_ac_uk/Ej7QTvDUlbdLki4LWYzCC_sBBjy9nIXoC59r5BFXlOYqbg?e=fjHnki}
	
	\item DOI/bib finder: 
	\begin{itemize}
		\item \url{https://dblp.org}
		\item \url{https://search.crossref.org/}
	\end{itemize}
\end{itemize}


\section*{ToDo (\textit{Chidimma})}
\begin{itemize}
	\item Finding more tools: Overlooked areas \textit{Threat Modelling} and \textit{Post-Exploitation} (\textit{Password Cracking} in particular)
	\item \begin{itemize}
		\item \url{https://dblp.uni-trier.de/search/publ?q=threat%24%20modelling%24}
		\item \url{https://dblp.uni-trier.de/search/publ?q=automated%24%20threat%24%20modelling%24}
		\item \url{https://dblp.uni-trier.de/search?q=post%24%20exploitation%24}
		\item \url{https://dblp.uni-trier.de/search/publ?q=password%24%20cracking%24}
		
	\end{itemize}
	\item Classify new tools (\textit{Paolo can help})
	\item Adding more tools descriptions after classification
	
\end{itemize}

